Bayesian Social Influence in the Online Realm

Our opinions, which things we like or dislike, depend on the opinions of those around us. Nowadays, we are influenced by the opinions of online strangers, expressed in comments and ratings on online platforms. Here, we perform novel "academic A/B testing" experiments with over 2,500 participants to measure the extent of that influence. In our experiments, the participants watch and evaluate videos on mirror proxies of YouTube and Vimeo. We control the comments and ratings that are shown underneath each of these videos. Our study shows that from 5$\%$ up to 40$\%$ of subjects adopt the majority opinion of strangers expressed in the comments. Using Bayes' theorem, we derive a flexible and interpretable family of models of social influence, in which each individual forms posterior opinions stochastically following a logit model. The variants of our mixture model that maximize Akaike information criterion represent two sub-populations, i.e., non-influenceable and influenceable individuals. The prior opinions of the non-influenceable individuals are strongly correlated with the external opinions and have low standard error, whereas the prior opinions of influenceable individuals have high standard error and become correlated with the external opinions due to social influence. Our findings suggest that opinions are random variables updated via Bayes' rule whose standard deviation is correlated with opinion influenceability. Based on these findings, we discuss how to hinder opinion manipulation and misinformation diffusion in the online realm.

==> include2/survey2_basic_tab.tex <==
\begin{tabular}{c|c|ccc|ccc|c|c}
\toprule
& & \multicolumn{3}{c|}{Comments} & \multicolumn{3}{c|}{Thumbs} & \\
  Survey &                   Video &  CPos &  CNeut &  CNeg &    TUp &  TDown & TFraction &    Views &                                                        Link to the original \\
\midrule
         &       Video 1 (htc add) &    17 &     30 &    47 &  110.0 &   31.0 &      0.78 &  147,273 &  \href{http://youtu.be/dwGGdM3Nj08}{dwGGdM3Nj08} \\
         &   Video 2 (lamborghini) &    14 &      1 &     5 &   41.0 &   28.0 &      0.59 &   76,675 &  \href{http://youtu.be/Pc7XHHCjtJI}{Pc7XHHCjtJI} \\
         &  Video 3 (girl singing) &    37 &     15 &    37 &  663.0 &  525.0 &      0.56 &  120,938 &  \href{http://youtu.be/5JKJhY15NNA}{5JKJhY15NNA} \\
 Prelim. &   Video 4 (supermarket) &     5 &      3 &    15 &   60.0 &   45.0 &      0.57 &   25,892 &  \href{http://youtu.be/VqGaHxC3Zbg}{VqGaHxC3Zbg} \\
         &    Video 5 (google car) &     2 &      7 &    10 &   50.0 &      - &       nan &        - &          \href{http://youtu.be/9261909}{9261909} \\
         &    Video 6 (stride add) &     8 &      8 &     3 &  221.0 &      - &       nan &        - &        \href{http://youtu.be/23061242}{23061242} \\
         &          Video 7 (ipad) &    33 &     14 &    13 &  842.0 &      - &       nan &        - &        \href{http://youtu.be/11480457}{11480457} \\
\hline
         &        Video 8 (cancer) &    19 &     10 &     8 &  695.0 &      - &       nan &        - &        \href{http://youtu.be/54668275}{54668275} \\
\bottomrule
\end{tabular}



==> sec_model-formulation.tex <==

In this section, we derive the logit model based on a Bayesian theory of social influence. 
Then, we explain the details of the model of sub-populations, that is a mixture of logit models introduced in the main text. We describe in detail model selection, the characteristics of the best models, and how the confidence intervals are computed.
%In the main text, we use this model to introduce the microscopic model, with which we infer influenceability of each participant, and the macroscopic model of sub-populations, which parsimoniously explains our experimental result. The microscopic model treats each individual separately, whereas the macroscopic model assumes that the individuals are indistinguishable and belong to certain sub-populations.

\subsection{The Derivation of Logit Model}

The derivation of the model follows the steps of Perez-Escudero et al.~\cite{Perez-Escudero2011Collective}, however, its interpretation is adapted to the setting of opinion formation. 
We consider liking or disliking a video as options that an individual may choose from, equivalent to having a positive or negative opinion about the video.
Each individual estimates the probability that liking a video is a good option using her prior information ($C$) and new social information ($B$), i.e.,
$P(+|C,B)$,
where $+$ stands for a positive opinion and the probability of a negative opinion is $P(-|C,B) = 1- P(+|C,B)$. From Bayes' theorem, we have
\begin{equation}
P(+|C,B) = \frac{P(B|+,C)P(+|C)}{P(B|-,C)P(-|C)+P(B|+,C)P(+|C)}.
\label{eq:Bmodel_Btheorem}
\end{equation}
By dividing numerator and denominator by the numerator we can rewrite it as
\begin{equation}
P(+|C,B) = \frac{1}{1+aS},
\label{eq:Bmodel_structure}
\end{equation}
where
\begin{equation}
\tilde{a} = \frac{P(-|C)}{P(+|C)}
\label{eq:non-social_term}
\end{equation}
and
\begin{equation}
\tilde{S} = \frac{P(B|-,C)}{P(B|+,C)}.
\label{eq:social_term0}
\end{equation}
%Since $\tilde{a}$ contains only prior information and the term $\tilde{S}$ contains all social information we refer to them as the \textit{prior opinion} and the \textit{social influeceability}, respectively. 
% paramter a
%The prior opinion represents the private preference for each video. 
%If $\tilde{a}>1$ the individual has a preference for negative opinion, and if $\tilde{a}<1$ for positive opinion.

% independent opinions assumption
We assume that each participant does not exploit the correlations among others' opinion, but instead assumes the opinions to be independent of each other. This strong assumption allows to derive a simple explicit expression that has been shown, for animals, to be a good approximation of the model including dependencies \cite{Perez-Escudero2011Collective}. 
Under this assumption $P(B|+,C) = Z \prod_{i=1}^{N}P(b_i|+,C)$, where $B$ is the set of $N$ comments read by the individual and $b_i$ is the opinion expressed in the comment $i$. $Z$ is a combinatorial term counting the number of possible comment sequences that lead to the set of comments $B$. A corresponding substitution in Equation \ref{eq:social_term0} gives
\begin{equation}
\tilde{S} = \prod_{i=1}^{N} \frac{P(b_i|-,C)}{P(b_i|+,C)}.
\label{eq:social_term1}
\end{equation}

As in the design of our experiments, we assume that each comment can be categorized as positive ($\beta_+$), negative ($\beta_-$), or neutral ($\beta_0$); consequently $N = n_+ + n_- + n_0$. Then,
\begin{equation}
\tilde{S} = \prod_{k \in \{ +,-,0 \} } \tilde{s}_{k}^{n_{k}}
\label{eq:social_term2}
\end{equation}
where
\begin{equation}
\tilde{s}_k = \frac{P(\beta_k|-,C)}{P(\beta_k|+,C)}
\label{eq:socia_subterm}
\end{equation}
With this expression for the social term we write Equation \ref{eq:Bmodel_structure} as
\begin{equation}
P(Y|C,B) = (1+\tilde{a} \tilde{s}_{+}^{n_+}\tilde{s}_{-}^{n_-}\tilde{s}_{0}^{N-n_{+}-n_{-}})^{-1}
\label{eq:Bmodel0}
\end{equation}

%\pms{This paragraph seem out of context to me}
%We assume that the private opinion of each video can be biased towards a positive or negative opinion. This assumption implies that in general $P(+|C) \neq P(-|C)$ and then $a \neq 1$ for each video. We can interpret that if $a>1$ the private opinion of each individual is biased towards negative values, and if $a<1$ the private opinion is biased towards positive values.

Next, we assume that neutral comments do not add any information. Thus, $P(\beta_0|-,C)=P(\beta_0|+,C)$ and $\tilde{s}_0 = 1$. Also, we assume that the influence of different types of comments is symmetrical, i.e., a positive comment negates a negative comment. This implies that $P(\beta_+|+,C)=P(\beta_-|-,C)$ and $P(\beta_+|-,C)=P(\beta_-|+,C)$. Considering that
\begin{equation}
\begin{aligned}
&\tilde{s}_- = \frac{P(\beta_-|-,C)}{P(\beta_-|+,C)}, \hspace{0.5cm} 
&\tilde{s}_+ = \frac{P(\beta_+|-,C)}{P(\beta_+|+,C)}
\end{aligned}
\label{eq:social_subterms}
\end{equation}
we can substitute these terms with $\tilde{s} \equiv \tilde{s}_- = 1/\tilde{s}_+$. Applying it to Equation \ref{eq:Bmodel0} gives the probability of positive opinion
\begin{equation}
P(+|\Delta n,\tilde{s},\tilde{a}) \equiv P_+(\Delta n,\tilde{s},\tilde{a}) = \frac{1}{1 + \tilde{a} \tilde{s}^{-\Delta n}}
\label{eq:Bmodel_symmetric}
\end{equation}
where $\Delta n = n_+ - n_-$.
%\pms{This paragraph sounds too complex. Could we simplify this? In fact, one or two sentences may be enough...
%To understand the meaning of the parameter $\tilde{s}$, let us consider the case of negative comments. $\tilde{s} = \frac{P(\beta_-|-,C)}{P(\beta_-|+,C)}$ can be interpreted as the probability that somebody writes a negative comment when the participant does not like the video, over the probability that somebody writes a positive comment when the participant likes the video. First, if the participant thinks that the viewers that wrote the comments have the same opinion (the participant agrees with the comments) $P(\beta_-|-,C)=1$ and  $P(\beta_-|+,C)=0$, consequently $\tilde{s}_- = \infty$ (social participant). Second, if the participant thinks that the viewers that wrote the comments do not have the same opinion (the participant does not agree with the comments) $P(\beta_-|-,C)=0$ and  $P(\beta_-|+,C)=1$, consequently $\tilde{s}_- = 0$ (anti-social participant). Finally, if the participant thinks that the comments of other viewers are not related to his own opinion about the video (the participant has no opinion about the comments) $P(\beta_-|-,C)=P(\beta_-|+,C)$, consequently $\tilde{s}= 1$ (no-social participant). 
%}
We have so far only considered the perceptual stage of decision-making, in which each participant estimates the probability that liking or not the video is a good option. Whether the video is liked or not is decided by a decision rule. Evidence for animals and humans suggests that individuals use a decision rule called probability matching \cite{Behrend1961Probability,Kirk1965Probability,Wozny2010Probability,Perez-Escudero2011Collective,Arganda2012common}. According to this rule, an individual chooses an option with a probability that is equal to the probability that this option is a good option. Thus, in our setting, the probability of positive opinion
\begin{equation}
P_+(\Delta n,\tilde{s},\tilde{a}) = \frac{1}{1+ \tilde{a} \tilde{s}^{-\Delta n}} = \frac{1}{1+ \exp( -a - s \Delta n ) },
\label{eq:model_logistic}
\end{equation}
where $a = -\ln(\tilde{a})$ and $s = \ln(\tilde{s})$ are parameters of a logistic function. We refer to these parameters as \textit{prior opinion} $a$ and \textit{social infleunceability} $s$. 
The prior opinion represents the private preference for each video. 
If $a>0$ the individual has a preference for positive opinion, and if $a<0$ for negative opinion.
The influenceability decides how much prior opinion changes under social influence. By analogy to the notion of prior opinion, we refer to $a+s\Delta n$ as \textit{posterior} opinion.
%
%The parameter $s$ corresponds to the slope of the dependence $P_+(\Delta n)$, while the ratio $a/s$ determines the center of the dependence, namely $P_+(\Delta n^\ast=a/s) = 0.5$. In contrast with $\tilde{a}$ and $\tilde{s}$, the parameters $a$ and $s$ impact the probability anti-symmetrically with respect to the center of symmetry at $\Delta n^\ast$, namely: $P_+(\Delta n - \Delta n^\ast|a,s) = P_+( -\Delta n - \Delta n^\ast |a,-s))$. 

\subsection{The Derivation of Beta-Binomial Model}



==> sec_models-micro-mle.tex <==
%% intro
%If the model of two sub-populations is correct, then we shall be able to identify strongly and weakly influenced participants of the experiment. 
%Also, we can aim to generalize this model by assuming that instead of sub-populations there is a continuous distribution of influenceability among individuals. In such case, we should be able to infer influenceability of each individual.
%Here, we achieve that with two different methods, namely: i) we use maximal likelihood estimation to infer the influenceability directly and ii) we exploit expectation-maximization to infer to which sub-population, non-social or social, belongs each individual.
%In both cases, we estimate the influenceability of each participant of our experiment. At the end of this section, we measure correlations between influenceability and other characteristics of subjects.

\subsection{Individual Influenceability Model}
%\subsection{Individual influenceability model (A)}

% intro
Here, we introduce a microscopic model that directly assumes a different value of influenceability for each individual, reported in the main text. 
% formulation 
%Note that we conducted $S=2$ parts of the experiment and that each survey was conducted for $U$ subjects and $V=7$ videos. The results of experiment are contained in the matrices $\pmb {\Delta n} \in \mathbb{R}^{S \times U \times V}$ and $\pmb y \in \mathbb{R}^{S \times U \times V}$, such that $\Delta n_{suv}$ is the difference in the number of comments read by individual $u$ when evaluating video $v$ of survey $s$, while $y_{suv} = H( \texttt{opinion} ) \in \{0,1\}$ is the Heaviside step function of the opinion expressed by the individual about the video.
We conducted the experiment for $U$ subjects and $V$ videos. The results of experiment are contained in the matrices $\pmb {\Delta n} \in \mathbb{R}^{U \times V}$ and $\pmb y \in \mathbb{R}^{U \times V}$, such that $\Delta n_{uv}$ is the difference in the number of comments read by individual $u$ when evaluating video $v$, while $y_{uv} = H( \texttt{opinion} ) \in \{0,1\}$ is the Heaviside step function of the opinion expressed by the individual about the video.
In this model, we assume that the prior opinion $a_v$ depends only on the video and captures its global quality and that the influenceability $s_u$ depends only on individual.
Under this model, the joint probability of data is
\begin{equation}
P_+^{uv} = \frac{1}{ 1+ \exp( -a_{v} - s_{u} \Delta n_{uv} ) } 
\end{equation}
\begin{equation}
\begin{split}
P(\pmb {\Delta n}, \pmb y) = \prod_{u=1}^U   \prod_{v=1}^V    
\left( P_+^{uv} \right)^{y_{uv}} 
\left( 1-P_+^{uv} \right)^{1-y_{uv}}.
\end{split}
\end{equation}

This model has a total of $(U+V)$ parameters. We fit these parameters by finding the maximum of the log-likelihood $\log \left( P(\pmb {\Delta n}, \pmb y) \right)$ using L-BFGS-B algorithm. We initialize all parameters with random values drawn from standard normal distribution. Independently of the initial values of the parameters, the algorithm converges to the global maximum, i.e., to the same global solution. 

We show the result of fitting this model in Figure~\ref{fig:modela-mainpop}. The measured running probability remains within $95\%$ confidence interval of the model. The model fits the data well at the level of the whole population, even though it essentially fits a logistic function separately for every individual. To illustrate it, we split the participants by the inferred values of their influenceability. 
The distribution of influenceability, shown in Figure~\ref{fig:dist-infl}, resembles a normal distribution and it is significantly positively skewed ($\gamma=6.7$, $p=0$).
For the purpose of illustration, we assign all participants with $s_u \leq 0$ to the low-influenceability group, whereas all subjects with $s_u > 0$ to the high-influenceability group. We plot the probability of positive opinion separately for each group and for each video (Figure~\ref{fig:modela-subpops}). We note that the model fits the measurements for each group remarkably well, since it fits the Bayesian decision-making model for each participant separately, while maintaining the prior opinion constant across all individuals and dependent on the video to describe the overall quality of the video. 
%In the main text, we report the distribution of influenceability inferred for each individual, as well as the versions of Figures~\ref{fig:modela-mainpop} and~\ref{fig:modela-subpops} that are collapsed for all videos.



\begin{figure*}[htb!]
\centering
\centerline{\subfigure{\includegraphics[width=1.05\textwidth]{figs2/model-rev-lbfgs-sp3-var20_expv_n5_ord-name_pubmflt_dnc-avg-100_binary_mainpop}}}
\centerline{\subfigure{\includegraphics[width=1.05\textwidth]{figs2/model-rev-lbfgs-sp3-var20_exp3_n5_ord-name_pubmflt_dnc-avg-100_binary_mainpop}}}
\caption{
Probability of positive opinion versus the difference in the number of positive and negative comments read by a subject. Blue points correspond to the moving average over $100$ measurements. The model applied to the finite real data expects the running average in the gray area marking $99\%$ confidence interval. The black line is the model applied to an infinite data.
}
\label{fig:modela-mainpop}
\end{figure*}


\begin{figure}[hbtp]
\centering
\subfigure{\includegraphics[width=0.3\textwidth]{figs2/pub_distro_inflity__var20}}
\caption{(A) The distribution of influenceability of individuals with negative (green) and positive (red hatched) influenceability.}
\label{fig:dist-infl}
\end{figure}

\begin{figure*}[htb!]
\centering
\centerline{\subfigure{\includegraphics[width=1.05\textwidth]{figs2/model-rev-lbfgs-sp3-var20_expv_n5_ord-name_pubmflt_dnc-avg-100_binary_subpops}}}
\centerline{\subfigure{\includegraphics[width=1.05\textwidth]{figs2/model-rev-lbfgs-sp3-var20_exp3_n5_ord-name_pubmflt_dnc-avg-100_binary_subpops}}}
\caption{
\pms{Change to newer figures}
Probability of positive opinion versus the difference in the number of positive and negative comments read by a subject. The green points are for subjects with low (negative) influenceability, whereas red points are for participants with high (positive) influenceability. The corresponding components of the model are marked with red and green lines.
}
\label{fig:modela-subpops}
\end{figure*}

%\begin{figure}[hbtp]
%\centering
%\subfigure{\includegraphics[width=0.3\textwidth]{figs/pub_distro_influenceability_var20}}
%\subfigure{\includegraphics[width=0.3\textwidth]{figs/pub-mainpop-dnc_collapsed-var20}}
%\subfigure{\includegraphics[width=0.3\textwidth]{figs/pub-subpops-dnc_collapsed-var20}}
%\caption{(A) The distribution of influenceability of participants with negative (green) and positive (red hatched) influenceability.
%(B and C) The probability of positive opinion versus the difference in the number of positive and negative comments read by the participants shifted by an offset that collapses plots for different videos. Figure (B) corresponds to an average over all users and videos. Figure (C) splits subjects having high infleunceability (red up triangles) from the ones with low influenceability (green down triangles).}
%\label{fig:modela-collapsed}
%\end{figure}




%\subsection{Influenceability versus characteristics of participants}
%\label{sec:infer}

%\begin{figure*}[htb]
%\begin{picture}(200,250)
%\centering
%\put(0,0){
%\centerline{\subfigure{\includegraphics[width=0.9\textwidth]{figs/pub-avg1_inflity_props_notrans_nt1000}}}
%}
%\put(5,170){\rotatebox{90}{Model A}}
%\put(5,52){\rotatebox{90}{Model B}}
%\end{picture}
%\caption{Various properties of subjects versus their influencaebility inferred with Model A (upper row) or with Model B (bottom row). The agreement with comments is self-reported by subjects and averaged over seven videos. The comments read are averaged over seven videos as well. The education is split in two categories: higher degree represented by 1 and no higher degree represented as 0. Error bars correspond to $95\%$ confidence interval (BCA).}
%\label{fig:inflity-props}
%\end{figure*}

%
%% results
%% two methods
%There is a strong correlation between the participants' influenceability inferred with the two methods (mean Spearman's $\rho=0.71$, $p<10^{-42}$). 
%Furthermore, subject's influenceability inferred with both methods is significantly correlated with her level of agreement ``with the feedback of other people'' averaged over videos ($\rho\in\{0.21,0.30\}$, $p<10^{-12}$; see Figures~\ref{fig:inflity-props}A and D). Thus, the inferred influencabilities are to some extent self-consistent.
%
%% other results
%Interestingly, two other characteristics of participants are significantly correlated with influenceability, independently from its inference method (see ``Describing sub-populations'' in the supplementary text). First, the more comments the subject tends to read, the less likely she is to be influenced by them ($\rho\in\{0.08,0.27\}$, $p\in\{0.02,10^{-5}\}$; see Figures~\ref{fig:inflity-props}B and E). Second, the more educated the participant is, the harder it is to influence her ($\rho\in\{0.09,0.10\}$, $p\in\{0.01,0.001\}$; see Figures~\ref{fig:inflity-props}C and F). 


% results
Furthermore, subject's influenceability is significantly correlated with her level of agreement ``with the feedback of other people'' averaged over videos ($\rho= 0.30$, $p<10^{-12}$. Thus, the inferred influencabilities are to some extent consistent with self-reported agreement of subjects.
% other results
Interestingly, two other characteristics of participants are significantly correlated with influenceability. First, the more comments the subject tends to read, the less likely she is to be influenced by them ($\rho = 0.08$, $p = 0.02$). Second, the more educated the participant is, the harder it is to influence her ($\rho = 0.10$, $p = 0.001$). 



==> sec_models-micro.tex <==
% intro
If the model of two sub-populations is correct, then we shall be able to identify strongly and weakly influenced participants of the experiment. 
Also, we can aim to generalize this model by assuming that instead of sub-populations there is a continuous distribution of influenceability among individuals. In such case, we should be able to infer influenceability of each individual.
Here, we achieve that with two different methods, namely: i) we use maximal likelihood estimation to infer the influenceability directly and ii) we exploit expectation-maximization to infer to which sub-population, non-social or social, belongs each individual.
In both cases, we estimate the influenceability of each participant of our experiment. At the end of this section, we measure correlations between influenceability and other characteristics of subjects.

\subsection{Individual influenceability model (A)}

% intro
Here, we introduce a microscopic model that directly assumes a different value of influenceability for each individual, reported in the main text. 
% formulation
Consider that the results of the experiment are stored in matrices $\pmb {\Delta n}$ and $\pmb y$, such that $\Delta n_{uv}$ is the difference in the number of comments read by individual $u$ when evaluating video $v$, while $y_{uv} = H( opinion ) \in \{0,1\}$ is Heaviside step function of the opinion expressed by the individual $u$ about video $v$.
Furthermore, in this model, we assume that the parameter $a_v$ captures the global quality of the video and the parameter $s_u$ is the influenceability of individual $u$.
Thus, the joint probability of $\pmb {\Delta n}$, $\pmb y$ can be written as
\begin{equation}
\begin{split}
P(\pmb {\Delta n}, \pmb y) = \prod_{u=1}^U   \prod_{v=1}^V    
\left( \frac{1}{1+ \exp( -a_{v} - s_{u} \Delta n_{uv} ) } \right)^{y_{uv}} 
\left( \frac{1}{1+ \exp( a_{v} + s_{u} \Delta n_{uv} ) } \right)^{1-y_{uv}},
\end{split}
\end{equation}
where $U$ is the total number of individuals and $V$ is the number of videos evaluated by each individual.

\begin{figure*}[htb!]
\centering
\centerline{\subfigure{\includegraphics[width=1.05\textwidth]{figs/model-fixedpi-var20_expv_n1000_ord-name_pubmflt_dnc-avg_mainpop}}}
\centerline{\subfigure{\includegraphics[width=1.05\textwidth]{figs/model-fixedpi-var20_exp3_n1000_ord-name_pubmflt_dnc-avg_mainpop}}}
\caption{Probability of positive opinion versus the difference in the number of positive and negative comments read by the participants. Blue circles correspond to the moving average over 150 measurements, whereas black line corresponds to the fitted Model A.}
\label{fig:modela-mainpop}
\end{figure*}

\begin{figure*}[htb!]
\centering
\centerline{\subfigure{\includegraphics[width=1.05\textwidth]{figs/model-fixedpi-var20_expv_n1000_ord-name_pubmflt_dnc-avg_subpops}}}
\centerline{\subfigure{\includegraphics[width=1.05\textwidth]{figs/model-fixedpi-var20_exp3_n1000_ord-name_pubmflt_dnc-avg_subpops}}}
\caption{Probability of positive opinion versus the difference in the number of positive and negative comments read by the participants. The green points are for subjects with low (negative) influenceability and the green line illustrates the corresponding component of the model, whereas red points and line are for participants with high (positive) influenceability.}
\label{fig:modela-subpops}
\end{figure*}

%\begin{figure}[hbtp]
%\centering
%\subfigure{\includegraphics[width=0.3\textwidth]{figs/pub_distro_influenceability_var20}}
%\subfigure{\includegraphics[width=0.3\textwidth]{figs/pub-mainpop-dnc_collapsed-var20}}
%\subfigure{\includegraphics[width=0.3\textwidth]{figs/pub-subpops-dnc_collapsed-var20}}
%\caption{(A) The distribution of influenceability of participants with negative (green) and positive (red hatched) influenceability.
%(B and C) The probability of positive opinion versus the difference in the number of positive and negative comments read by the participants shifted by an offset that collapses plots for different videos. Figure (B) corresponds to an average over all users and videos. Figure (C) splits subjects having high infleunceability (red up triangles) from the ones with low influenceability (green down triangles).}
%\label{fig:modela-collapsed}
%\end{figure}


In total, this model has $(U+V)$ parameters that need to be fitted at once. We fit these parameters by finding the maximum of the log-likelihood of $P(\pmb {\Delta n}, \pmb y)$. To that end, we use L-BFGS-B. We initialize all the parameters with a standard normal distribution. Independently of the initial values of the parameters, the method converges to the global maximum, i.e., to the same global solution. 

We show the result of fitting this model in Figure~\ref{fig:modela-mainpop}. The measured running probability remains within $95\%$ confidence interval of the model. The model fits well the data at the level of the whole population, even though it essentially fits a sigmoid function for every participant of the experiment. To show it, we split the participants by the value of influenceability $s_u$ inferred for each of them by the model. We assign all participants with $s_u \leq 0$ to the low influenceability sub-population, whereas all subjects with $s_u > 0$ to the high influenceability sub-population. We plot the probability of positive opinion separately for each sub-population and for each video (Figure~\ref{fig:modela-subpops}). We note, that the model fits the two sub-populations remarkably well. This is to be expected, since this approach fits the Bayesian decision-making model for each participant, while maintaining the parameters $a_v$, describing the quality of each video, constant for the whole population. In the main text, we report the distribution of influenceability inferred for each individual, as well as the versions of Figures~\ref{fig:modela-mainpop} and~\ref{fig:modela-subpops} that are collapsed for all videos.



\subsection{Sub-population membership model (B)}

Here, we introduce the microscopic model of sub-populations and infer sub-population membership of every individual using expectation maximization (EM). We define each sub-population as a set of individual who have the same characteristics, namely, the same values of parameters $a$ and $s$. An individual belonging to sub-population $k$ watching a video $v$ and seeing comments of valence $\Delta n_{uv}$ has the following probability of having a positive opinion about this video
\begin{equation}
P_{+}(n_{uv}) = \frac{1}{1+ \exp( -a_{kv} - s_{k} \Delta n_{uv} ) }.
\end{equation}
Our goal is to assign all individuals to one of the sub-populations by performing EM for a mixture of such logistic functions. In general, EM optimizes log-likelihood of a statistical model with latent variables. 
In our case, the latent variables encode sub-population membership of an individual.
Consider a matrix of latent variables $\pmb z$ whose elements $z_{uk} \in \{0,1\}$ tell us if individual $u$ belongs to sub-population $k$ and $z_u$ is an one-of-$k$ variable (every person is assigned to exactly one sub-population). The joint probability of $\pmb {\Delta n}$, $\pmb y$, and $\pmb z$ is
\begin{equation}
\begin{split}
P(\pmb {\Delta n}, \pmb y, \pmb z) = \prod_{u=1}^U \prod_{k=1}^K \left( \pi_k \prod_{v=1}^V    
\left( \frac{1}{1+ \exp( -a_{kv} - s_{k} \Delta n ) } \right)^{y_{uv}} \right.\\
\left. \left( \frac{1}{1+ \exp( a_{kv} + s_{k} \Delta n ) } \right)^{1-y_{uv}}
\right)^{z_{uk}},
\end{split}
\end{equation}
where $U$ is the total number of individuals, $V$ is the total number of videos per subject, $K$ is the total number of sub-population, and $\pi_k$ is the probability that an individual belongs to sub-population $k$, $a_{vk}$ and $s_k$ are the group-specific parameters of our model. 
%This constitutes complete-data likelihood function. However, $\pmb z$ is a latent variable and it is not observed. Thus, we need to resort to expectation, with respect to the posterior distribution of the latent variable, of the complete-data log-likelihood:
The expected value, with respect to the posterior distribution of the latent variable, of the complete-data log-likelihood is
\begin{equation}
\begin{split}
\mathbb{E}_{\pmb z} [\ln P(\pmb {\Delta n}, \pmb y, \pmb z)] = \sum_{u=1}^U \sum_{k=1}^K \gamma({z_{uk}}) 
\left( \ln \pi_k +  \sum_{v=1}^V \left(
y_{uv} \ln( \frac{1}{1+ \exp( -a_{kv} - s_{k} \Delta n ) }) + \right. \right. \\
\left. \left. (1-y_{uv}) \ln( \frac{1}{1+ \exp( a_{kv} + s_{k} \Delta n ) }) 
\right) \vphantom{\sum_{k=1}^K} \right),
\label{eq:p-expectation}
\end{split}
\end{equation}
where $\gamma({z_{uk}})$ is the responsibility of sub-population $k$ for individual $u$, i.e.,
\begin{equation}
\gamma({z_{uk}}) = 
\frac{
\pi_k \prod_{v=1}^V    
\left( \frac{1}{1+ \exp( -a_{kv} - s_{k} \Delta n ) } \right)^{y_{uv}} 
\left( \frac{1}{1+ \exp( a_{kv} + s_{k} \Delta n ) } \right)^{1-y_{uv}}
}{
\sum_{k=1}^K \left( \pi_k \prod_{v=1}^V    
\left( \frac{1}{1+ \exp( -a_{kv} - s_{k} \Delta n ) } \right)^{y_{uv}} 
\left( \frac{1}{1+ \exp( a_{kv} + s_{k} \Delta n ) } \right)^{1-y_{uv}}
\right) }.
\label{eq:responsibility}
\end{equation}
The responsibilities $\gamma({z_{uk}})$ take values from 0 to 1 and $\gamma({z_{u0}}) + \gamma({z_{u1}}) = 1$. A value of $\gamma({z_{uk}})$ that is close to $1$ means that the behavior of individual $u$ is explained by the sub-population $k$, while a value that is close to $0$ means that the behavior of that individual must be explained by a different sub-population. 

The EM algorithm maximizes the expected complete-data log-likelihood by finding optimal values of the parameters $a_{vk}$, $s_k$, and $\pi_{k}$, and by computing the expected value of $z_{uk}$, namely the responsibilities $\gamma({z_{uk}})$. In the E step, we compute the responsibilities $\gamma({z_{uk}})$ using initial or last-iteration values of the parameters $a_{vk}$, $s_k$, and $\pi_{k}$. In the M step, we keep the responsibilities fixed and maximize Eq.~\ref{eq:p-expectation} with respect to the parameters $a_{vk}$, $s_k$, and $\pi_{k}$. The closed form solution for the optimal value of the parameter $\pi_{k}$ is
\begin{equation}
\pi_k = \frac{N_k}{N}, \hspace{5mm} \text{where:} \hspace{5mm} 
N_k = \sum_{u=1}^U \gamma({z_{uk}}), \hspace{5mm} N = \sum_k N_k.
\label{eq:pi}
\end{equation}
%We could not obtain closed form solutions for the other parameters. Note, however, that the optimization of the complete-data log-likelihood corresponds to the optimization of a mixture of logistic functions. Thus, to solve this optimization problem we can use numerical methods. Here, we use L-BFGS algorithm to find the optimal values of the parameters $a_{vk}$ and $s_k$. 
To obtain values of the remaining parameters we use L-BFGS-B algorithm to find the optimal values of the parameters $a_{vk}$ and $s_k$. 
This closes the M step of the EM algorithm. We repeat the E and M steps until convergence of the log-likelihood. 


% inference
Following the parsimonious model of sub-populations from the main text, we fix $K=2$ and $s_1=0$. Also, we fix $p_1=0.5$, to force a balanced ratio of social and non-social individuals for the purpose of the presentation. To find the remaining parameters, we fit our model using EM approach separately to the two parts of our experiment \footnote{In each part of the experiment a different set of videos has been evaluated}. 
This method has only $(V+1)$ parameters. However, the complexity of this model is governed by the number of latent variables encoding the responsibilities $\gamma({z_{uk}})$ of sub-population $k$ for individual $u$, that is $U$ latent parameters. These latent parameters are different from normal parameters, because they take constrained values from 0 to 1, cannot be observed directly, and are inferred differently than normal parameters.
As before, we initialize all parameters with a standard normal distribution.
We run the EM algorithm $1000$ times for each of the two parts of the experiment. 
The fitting with EM is not as consistent as the MLE model. Each time a slightly different solution is found. In the remainder, we report results that are averaged over $50$ solutions corresponding to the highest log-likelihoods. \pms{Not done yet; most figures are for the run with the highest log-likelihood now.}



\begin{figure*}[htb!]
\centering
\centerline{\subfigure{\includegraphics[width=1.05\textwidth]{figs/model-fixedpi-var3_expv_n1000_ord-name_pubmflt_dnc-avg_mainpop}}}
\centerline{\subfigure{\includegraphics[width=1.05\textwidth]{figs/model-fixedpi-var3_exp3_n1000_ord-name_pubmflt_dnc-avg_mainpop}}}
\caption{Probability of positive opinion versus the difference in the number of positive and negative comments read by the participants. Blue circles correspond to the moving average over 150 measurements, whereas black line corresponds to the fitted Model A.}
\label{fig:modelb-mainpop}
\end{figure*}

\begin{figure*}[htb!]
\centering
\centerline{\subfigure{\includegraphics[width=1.05\textwidth]{figs/model-fixedpi-var3_expv_n1000_ord-name_pubmflt_dnc-avg_subpops}}}
\centerline{\subfigure{\includegraphics[width=1.05\textwidth]{figs/model-fixedpi-var3_exp3_n1000_ord-name_pubmflt_dnc-avg_subpops}}}
\caption{Probability of positive opinion versus the difference in the number of positive and negative comments read by the participants. The green points are for subjects with low (negative) influenceability and the green line illustrates the corresponding component of the model, whereas red points and line are for participants with high (positive) influenceability.}
\label{fig:modelb-subpops}
\end{figure*}

\begin{figure}[hbtp]
\centering
\subfigure{\includegraphics[width=0.3\textwidth]{figs/pub_distro_influenceability_var3}}
\subfigure{\includegraphics[width=0.3\textwidth]{figs/pub-mainpop-dnc_collapsed-var3}}
\subfigure{\includegraphics[width=0.3\textwidth]{figs/pub-subpops-dnc_collapsed-var3}}
\caption{(A) The distribution of influenceability of individuals with negative (green) and positive (red hatched) influenceability.
(B and C) The probability of positive opinion versus the difference in the number of positive and negative comments read by the participants shifted by an offset that collapses plots for different videos. Figure (B) corresponds to an average over all individuals and videos. Figure (C) splits subjects having high infleunceability (red up triangles) from the ones with low influenceability (green down triangles).}
\label{fig:modelb-collapsed}
\end{figure}

\subsubsection*{Results}

% fit
We show how this model fits the measurements separately for each video (Figure~\ref{fig:modelb-mainpop}). We note that this model fits the data not as well as the parsimonious model or the individual influenceability model. For several videos, the measurements are beyond the $95\%$ confidence interval of the model.
% split
Next, we split the participants into two sub-population by checking which cluster they are associated with (Figure~\ref{fig:modelb-subpops}). The participants that have $\gamma({z_{uk}}) > 0.5$ for the group $k$ with non-zero influenceability are associated with the social sub-population. The participants that have $\gamma({z_{uk}}) \leq 0.5$ are associated with non-social sub-population. Most of subjects belong to the non-social sub-population (around $70\%$ of subjects), while a significant number of users belong to the social sub-population (remaining $30\%$ of subjects), what is consistent with the predictions of our macroscopic parsimonious model of sub-populations.
% results
We see that the effect of manipulation is barely visible for the non-social sub-population and considerable for the social sub-population (compare green and red points in Figure~\ref{fig:modelb-subpops}). However, there are some exceptions. Namely, for some videos the effect of manipulation is visible also for the non-social sub-population (see Figures~\ref{fig:modelb-subpops}F-G) and for some videos it is not visible for the social sub-population (see Figure~\ref{fig:modelb-subpops}F). Apparently, inferring membership to sub-populations is not is not as accurate as direct inference of influenceability.

%This happens, because the parameter $s$ does not only depend on the user, but also on the video that the user is consuming. In other words, a user may have a strong private perception about a video (e.g., she is an expert on the topics of the video) and it is difficult to manipulate her opinion about that video, however, the same user may have weaker private perception about another video (e.g., she is not an expert on other topics) and so it is easy to manipulate her opinion about this video. 

\subsubsection{Collapsing results for all videos}
Next, we collapse per-video plots by applying the transformation $\Delta \hat{n}_{uv} = \Delta n_{uv} - a_{uv}/s_{uv}$ for each answer of every individual. This transformation centers the plots for different videos by subtracting its expected center on the x-axis. 
In the case of sub-populations, to obtain the influenceability we multiply $\gamma (z_{uk})$ by the corresponding influenceability $s_k$ and average it over different sub-populations $k$ (Figure~\ref{fig:modelb-collapsed})).
%for each subject we pick the influenceability of the sub-population that he is more associated with, i.e., for which she has higher $\gamma (z_{uk})$ ( (Figure~\ref{fig:modelb-collapsed})). 
%
We note that the data lays in the $95\%$ confidence interval of the model. However, there is a noticeable difference between the confidence interval and the theoretical model for infinite data. This stems from several reasons. First, the confidence intervals are for finite data. Second, the values of the parameters may be not accurate, so the transformation that is supposed to center the data is not precise either, because it depends on these parameters. Third, there may be correlations between transformed x-axis values $\Delta \hat{n}_{uv}$ of each individual and the parameters of these subjects.  
Finally, we notice that this distribution of influenceability is different that the distribution of individual influenceability shown in the main text. This difference arises because the two methods infer influenceability in different ways.


%However, the fitting with EM is not as consistent as the MLE model. There are two reasons for that. First, EM fits directly to the measurements, while our prior approaches fit to the running average. Thus, EM is subject to a large amount of noise present in the measurements. Second, EM deals with a much higher number of parameters, due to inclusion of the responsibilities that encode the sub-populations. Thus, we use EM only for clustering users into strongly and weakly social groups, whereas for fitting the plotted curves we use the prior approaches.

%Potentially, we could explore also the possibility of having video-dependent herding parameters $s_{kv}$. In such case, these parameters would represent how convincing are the comments for each of the videos. However, I think this may be already too complex for our study and we should decide what we want to focus on in the paper and what should be overall message of the paper. If the message is that there are social and non-social users, then $s_{k}$ is better model, because it is simpler and to the point.




\subsection{Influenceability versus characteristics of participants}
\label{sec:infer}

\begin{figure*}[htb]
\begin{picture}(200,250)
\centering
\put(0,0){
\centerline{\subfigure{\includegraphics[width=0.9\textwidth]{figs/pub-avg1_inflity_props_notrans_nt1000}}}
}
\put(5,170){\rotatebox{90}{Model A}}
\put(5,52){\rotatebox{90}{Model B}}
\end{picture}
\caption{Various properties of subjects versus their influencaebility inferred with Model A (upper row) or with Model B (bottom row). The agreement with comments is self-reported by subjects and averaged over seven videos. The comments read are averaged over seven videos as well. The education is split in two categories: higher degree represented by 1 and no higher degree represented as 0. Error bars correspond to $95\%$ confidence interval (BCA).}
\label{fig:inflity-props}
\end{figure*}


% results
% two methods
There is a strong correlation between the participants' influenceability inferred with the two methods (mean Spearman's $\rho=0.71$, $p<10^{-42}$). 
Furthermore, subject's influenceability inferred with both methods is significantly correlated with her level of agreement ``with the feedback of other people'' averaged over videos ($\rho\in\{0.21,0.30\}$, $p<10^{-12}$; see Figures~\ref{fig:inflity-props}A and D). Thus, the inferred influencabilities are to some extent self-consistent.

% other results
Interestingly, two other characteristics of participants are significantly correlated with influenceability, independently from its inference method (see ``Describing sub-populations'' in the supplementary text). First, the more comments the subject tends to read, the less likely she is to be influenced by them ($\rho\in\{0.08,0.27\}$, $p\in\{0.02,10^{-5}\}$; see Figures~\ref{fig:inflity-props}B and E). Second, the more educated the participant is, the harder it is to influence her ($\rho\in\{0.09,0.10\}$, $p\in\{0.01,0.001\}$; see Figures~\ref{fig:inflity-props}C and F). 


